Improving Graph Neural Network Representations of Logical Formulae with Subgraph Pooling

Recent advances in the integration of deep learning with automated theorem proving have centered around the representation of logical formulae as inputs to deep learning systems. In particular, there has been a growing interest in adapting structure-aware neural methods to work with the underlying graph representations of logical expressions. While more effective than character and token-level approaches, graph-based methods have often made representational trade-offs that limited their ability to capture key structural properties of their inputs. In this work we propose a novel approach for embedding logical formulae that is designed to overcome the representational limitations of prior approaches. Our architecture works for logics of different expressivity; e.g., first-order and higher-order logic. We evaluate our approach on two standard datasets and show that the proposed architecture achieves state-of-the-art performance on both premise selection and proof step classification.

==> broader_impact.tex <==
\section{Statement of Broader Impact}

As our approach is capable of handling higher-order logic, we believe our work could be useful for more than just theorem proving. Any logic domain requiring the neural representation of formulae could use our approach as their embedding mechanism (e.g., for embedding DAG representations of HTN plans or SAT problems). Further, our approach is particularly useful where the complete context of a DAG at a node (i.e., the set of nodes above or below the node) are useful for understanding the node itself (e.g., the subgraph beneath a node in a formula's graph corresponds to a subformula). Thus, any domain for which that property holds (e.g., embedding dependency parses in NLP) could perhaps benefit from our method.

% DAGs are very general, common data-structures. Thus, we imagine the negative outcomes of our work would be in the tools used by malicious parties, who could possibly improve their systems (e.g., SAT solvers) that leverage DAG representations internally.

This work aims for improving the representation of DAG-based logical formulas. To the best of our knowledge, we do not believe that this work by itself has direct negative societal consequences. However, it could possibly be used by malicious parties to improve their systems (e.g., SAT solvers) that leverage DAG representations internally.

%In terms of However, if better embedded representations of DAGs w

% \textbf{EDITOR NOTE FROM ACHILLE: I'm not sure this last paragraph is really necessary -especially if we have a space issue}





==> conclusions.tex <==
\section{Conclusions}% and Future Work}

In this work, we introduced a novel method for computing neural representations of logical formulae that was designed with careful consideration to their unique structural properties. Our approach achieved new state-of-the-art performances on two standard datasets, despite the datasets involving different logical formalisms. We also showed how to easily  incorporate our method with an existing theorem prover as its premise selection mechanism; where its inclusion led to a 61.6\% improvement in terms of number of proofs found.

%An interesting future line of research could be in exploring the attention mechanism introduced in Section \ref{sec:dep_glstm}. One could see if different pairing operations than identicality (e.g., structural similarities derived from works like \cite{falkenhainer1989structure}) lead to more efficiency with better performance. One might also explore the effect that the initial node embedder has on the similarities computed by the attention mechanism. When using an MPNN for node embeddings, one might expect the attention mechanism to be computing local neighborhood similarity; however, when using a DAG LSTM, it is less obvious what type of similarity is being captured. Inspecting what the neural network learns to be the most useful subgraphs to match could lead to insights that produce new heuristics for proof guidance.

